He~I Emission in the Orion Nebula and Implications for Primordial Helium Abundance

We apply a recently developed theoretical model of helium emission to observations of both the Orion Nebula and a sample of extragalactic H II regions. In the Orion analysis, we eliminate some weak and blended lines and compare theory and observation for our reduced line list. With our best theoretical model we find an average difference between theoretical and observed intensities $<I_{predicted}/I_{observed}-1> = 6.5%$. We argue that both the red and blue ends of the spectrum may have been inadequately corrected for reddening. For the 22 highest quality lines, with $3499 {\AA}\le\lambda\le6678 {\AA}$, our best model predicts observations to an average of 3.8%. We also perform an analysis of the reported observational errors and conclude they have been underestimated. In the extragalactic analysis, we demonstrate the likelihood of a large systematic error in the reported data and discuss possible causes. This systematic error is at least as large as the errors associated with nearly all attempts to calculate the primordial helium abundance from such observations. Our Orion analysis suggests that the problem does not lie in the theoretical models. We demonstrate a correlation between equivalent width and apparent helium abundance of lines from extragalactic sources that is most likely due to underlying stellar absorption. Finally, we present fits to collisionless case-B He I emissivities as well as the relative contributions due to collisional excitations out of the metastable $2s {}^{3}S$ term.

==> response <==
Dear Editor,

Please find below our itemized responses to the referee's report.  Through private communication, the referee has revealed his identity to us, and I have added a statement thanking him explicitly for his review.  

Cheers,
Ryan Porter    

(1) In the introduction, it would be nice to cite a paper or two which emphasises the need for measurements of cosmological parameters, independent of the CMB results.  (An example would be:
\bibitem[Bridle et al.(2003)]{2003Sci...299.1532B} Bridle, S.~L., Lahav, O., Ostriker, J.~P., \& Steinhardt, P.~J.\ 2003, Science, 299, 1532 )

--Okay.  Cited Bridle et al. 2003.

(2) The analysis of the Orion spectrum is great.  I especially like the test of the assigned observational errors by comparing the ratios of lines from the same upper level.  It is disappointing that Esteban et al. did not perform a similar test in order to validate their error determinations. Since underestimates of errors are epidemic in this field I would like to see a sentence in the abstract indicating that this test was performed with the result that the reported errors had been underestimated.

--Added sentence to abstract.

(3) In Table 1, the HeI intensities, relative to H-beta (or 5876) for each of the three models, should be listed for completeness and reproducibility.

--Included intensities in Table 1.

(4) In Table 2, the observational uncertainties are reported as percentages in the last column.  It would be much more useful to report the observations, with the uncertainties, in standard form XX +/- YY.  Then the next column should report the differences in positive or negative standard deviations (instead of percentages).  Then it is immediately apparent which lines discrepant, and which are not.

--Made recommended changes.  In doing so, I discovered that I had made an error in the error analysis.  Errors are still large, but normal distribution now cannot be produced by scaling errors.  I changed the corresponding text accordingly, in particular adding a statement that the large standard deviations violate the Chebychev Inequality applicable to any statistical distribution with finite variance.

(5) In Figure 3, the line connecting 4p1P to 3s1S, which I believe is 1.508 microns, is labelled as FIR; I believe that it should be labelled at IR.

--Made change.

(6) The 3188+3889+4713+5876+7065 diagnostic appears to be quite useful. In its description, of the 5 possible decay paths, shouldn't 5 be "followed by emission of a photon at 5876 or
3889 or 7065"?

-Yes, made change.

(7) It would be useful to point out that for the overwhelming majority of HII region spectra, He I 3188 is not observed.  
This may inspire some new UVES proposals.  Although the line only 20% of 5876, there is significant extinction, and the throughput of UVES is down by a factor of 3 from nominal at 3200, it may still be possible to observe this line for some of the brightest targets (Magellanic Clouds).

--Added statement about observation of 3188.

(8) It should be stated why only the 33 new observations from
IT04 have been analyzed.  I think that this is probably because the presentation of the data are best and easiest to follow, but it should be stated explicitly.  Note that many of these new targets are not especially low metallicity and were observed to broadened the metallicity baseline.

--Specified that we use only the new ones ``for simplicity.''

(9) The analysis in Figures 6 and 7 is very similar to the analysis of the IT98 data by Skillman et al. (1998):
\bibitem[Skillman et al.(1998)]{1998SSRv...84..105S} (Skillman, E.~D., Terlevich, E., \& Terlevich, R.\ 1998, Space Science Reviews, 84, 105,) with identical results.  This work should be cited, as it shows that the flaws in the IT04 analysis are not new, but have been known for some time.

--Added a reference to Skillman et al. 1998 in the discussions of Figures 6 and 7.

(10) Of course, it doesn't make sense to assume a single EW for the He I lines for different targets.  These should be solved for on a per target basis, as was demonstrated by Olive & Skillman (2001): (\bibitem[Olive \& Skillman(2001)] {2001NewA....6..119O} Olive, K.~A., \& Skillman, E.~D.\ 2001, New Astronomy, 6, 119) and applied to these data in Olive & Skillman (2004).

--Added statement to this effect, including references to Olive & Skillman 2001 and 2004.

(11) I agree that the best way to address the underlying absorption problem may be to compare to theoretical models like Gonzalez Delgado et al.  You can cite the application of this technique in the Tremonti et al. (2004) paper:
(\bibitem[Tremonti et al.(2004)]{2004ApJ...613..898T} Tremonti, C.~A., et al.\ 2004, \apj, 613, 898).

--Added statement and reference to Tremonti et al. (2004).

(12) The proposed solution of replacing a cut-off in EW(H-beta) with a cut-off in the EW of individual He I lines is specious.  Since the He abundance is essentially identical for all of these targets, the two will be equivalent, except that one then throws away all of the lines except 5876.  Thus one throws away all of the information used to constrain things like density, temperature, and optical depth.  If I have misread this, and you are advocating using all of the He I lines to determine physical conditions, but then using only 5876 to determine the He I abundance, then this still is a step back from a "self-consistent" model as used in the Orion analysis.  Even following this suggestion does not result in the proposed trade from large systematic uncertainties to small random errors.  There are other systematic uncertainties which still dominate (i.e., the determination of the appropriate physical conditions). (see Peimbert et al. 2002:
(\bibitem[Peimbert et al.(2002)]{2002ApJ...565..668P} Peimbert, A., Peimbert, M., \& Luridiana, V.\ 2002, \apj, 565, 668) This suggestion does not merit a sentence in the abstract unless it is thought through more thoroughly.

--Removed sentence from abstract.  Changed suggested cutoff from 20Ang to 10Ang.  Added word additional to clarify that this cutoff would be in addition to an H-Beta cutoff.  Left statement about error tradeoff, but added sentence about other systematic uncertainties and reference to Peimbert et al. (2002).    

(13) My impression from Benjamin et al. (1999) was that solving for recombination emissivities and collisional contributions self-consistently produced differences from multiplying the two as suggested in the Appendix ("simply multiply the result").  I think that the appendix and Tables 4 and 5 are a valuable addition to the paper, but I also think that the point of self-consistency should be addressed.  After all, this is what CLOUDY does.  For figures 8 and 9 it should be noted that an ne of 100 and a Te above 15000K are typical of the HII regions used to derive the primordial helium abundance.  Here the differences are at least a few percent.  These represent minimum systematic errors.

--Added sentences to the beginning and end of appendix to address this.

